Towards Large-Scale AFQMC Calculations: Large Time Step Auxiliary-Field Quantum Monte Carlo

We report modifications of the ph-AFQMC algorithm that allow the use of large time steps and reliable time step extrapolation. Our modified algorithm eliminates size-consistency errors present in the standard algorithm when large time steps are employed. We investigate various methods to approximate the exponential of the one-body operator within the AFQMC framework, distinctly demonstrating the superiority of Krylov methods over the conventional Taylor expansion. We assess various propagators within AFQMC and demonstrate that the Split-2 propagator is the optimal method, exhibiting the smallest time-step errors. For the HEAT set molecules, the time-step extrapolated energies deviate on average by only 0.19 kcal/mol from the accurate small time-step energies. For small water clusters, we obtain accurate complete basis-set binding energies using time-step extrapolation with a mean absolute error of 0.07 kcal/mol compared to CCSD(T). Using large time-step ph-AFQMC for the N$_2$ dimer, we show that accurate bond lengths can be obtained while reducing CPU time by an order of magnitude.

==> tables/3UUDdis.tex <==
\begin{table}
\caption{\label{tab:3UUDdis}
The AFQMC energies of the stretched 3UUD cluster and its fragments, and the binding energies demonstrate that ph-AFQMC and ph$^{*}$-AFQMC are both size-consistent (all values are given in \unit{\hartree}).}
\begin{ruledtabular}
\begin{tabular}{l*{2}{d}}
Cluster             & \multicolumn{1}{c}{ph-AFQMC} & \multicolumn{1}{c}{ph$^{*}$-AFQMC}             \\ \hline
3UUD                & -228.82750(12)    & -228.82448(12)      \\
1-H$_2$O            &  -76.27576(4)     &  -76.27475(4)       \\
2-H$_2$O            &  -76.27580(4)     &  -76.27477(4)       \\
3-H$_2$O            &  -76.27585(4)     &  -76.27481(4)       \\ \hline
$E_b$               &    0.00009(14)    &    0.00015(14)
\end{tabular}
\end{ruledtabular}
\end{table}

==> tables/exchange.tex <==
\begin{table}
\caption{\label{tab:exchange} 
Summary of the methods for exchange energy evaluation with their computational scaling and corresponding memory requirements.
$N$ represents the number of basis functions, $N_g$ is the number of Cholesky vectors, $N_{\gamma}$ is number of reduced Cholesky vectors and $N_e$ is the number of electrons in the system.}
\begin{ruledtabular}
\begin{tabular}{llll}
Approach          & \multicolumn{1}{c}{Abbreviation}       & \multicolumn{1}{c}{Scaling} & \multicolumn{1}{c}{Storage} \\ \hline
Full ERI          & F-ERI              & $\mathcal{O}(N^4)$              & $\mathcal{O}(N^4)$   \\
Full Cholesky     & F-Chol             & $\mathcal{O}(NN_gN_e^2)$        & $\mathcal{O}(N^2N_g)$  \\
Reduced ERI       & R-ERI              & $\mathcal{O}(N^2N_e^2)$         & $\mathcal{O}(N^2N_e^2)$  \\
Reduced Cholesky  & R-Chol             & $\mathcal{O}(NN_{\gamma}N_e^2)$ & $\mathcal{O}(N^2N_{\gamma}) $  \\ 
\end{tabular}
\end{ruledtabular}
\end{table}

==> tables/heat_values.tex <==
\begin{table*}
\caption{\label{tab:heat_values} Total molecular energies (in Hartree units) for the HEAT set\cite{Tajti2004Heat} molecules at different levels of theory: ph-AFQMC\cite{Zhang2003Phaseless}, ph$^{*}$-AFQMC, CCSD(T), CCSDTQP\cite{Bomble2005Heat} and HCI\cite{Umrigar2016HeatBath,Sharma2017HeatBath}. All energies are calculated using the cc-pVDZ basis set. The last three rows of the table depict the root-mean-square deviation (RMSD), mean signed deviation (MSD), and mean absolute deviation (MAD).}
\begin{ruledtabular}
\begin{tabular}{l*{5}{d}}
Molecule            & \multicolumn{1}{c}{ph-AFQMC} & \multicolumn{1}{c}{ph$^{*}$-AFQMC} & \multicolumn{1}{c}{CCSD(T)} & \multicolumn{1}{c}{CCSDTQP} & \multicolumn{1}{c}{HCI} \\ \hline
H$_2$               & -1.16363(2)   & -1.16338(3)  & -1.163426   & -1.163426   & -1.163426   \\
CH                  & -38.37764(6)  & -38.37705(7) & -38.379655  & -38.380241  &             \\
CH$_2$              & -39.04181(5)  & -39.04150(6) & -39.041196  & -39.04165   &             \\
NH                  & -55.09087(5)  & -55.09077(7) & -55.097448  & -55.0917    &             \\
CH$_3$              & -39.71651(6)  & -39.71592(7) & -39.715543  & -39.71607   &             \\
NH$_2$              & -55.73265(6)  & -55.73222(8) & -55.732506  & -55.733076  &             \\
OH                  & -75.55854(6)  & -75.55837(8) & -75.559233  & -75.559689  &             \\
HF                  & -100.22933(7) & -100.2290(1) & -100.228131 & -100.228622 &             \\
H$_2$O              & -76.24249(8)  & -76.24167(9) & -76.241018  & -76.241649  & -76.241637  \\
NH$_3$              & -56.40334(7)  & -56.4024(1)  & -56.401913  & -56.402517  &             \\
C$_2$H              & -76.3999(2)   & -76.3986(2)  & -76.398558  & -76.401217  &             \\
CN                  & -92.4997(2)   & -92.4973(2)  & -92.488695  & -92.49276   & -92.492788  \\
C$_2$H$_2$          & -77.1118(2)   & -77.1092(2)  & -77.109249  & -77.110678  &             \\
CO                  & -113.0594(2)  & -113.0567(2) & -113.054431 & -113.055892 &             \\
HCN                 & -93.1912(2)   & -93.1881(2)  & -93.188321  & -93.18991   &             \\
N$_2$               & -109.2781(2)  & -109.2750(2) & -109.275298 & -109.277012 & -109.277005 \\  
HCO                 & -113.5778(2)  & -113.5757(2) & -113.575706 & -113.577384 &             \\
CF                  & -137.4764(1)  & -137.4754(2) & -137.474848 & -137.476019 &             \\
NO                  & -129.5970(2)  & -129.5945(2) & -129.597778 & -129.599737 &             \\
HNO                 & -130.1736(2)  & -130.1697(2) & -130.170989 & -130.172906 &             \\
O$_2$               & -149.9792(2)  & -149.9787(2) & -149.985684 & -149.987773 &             \\
HO$_2$              & -150.5606(2)  & -150.5603(2) & -150.558481 & -150.56038  &             \\ 
OF                  & -174.5004(2)  & -174.4998(2) & -174.497924 & -174.50009  &             \\
H$_2$O$_2$          & -151.1963(2)  & -151.1940(2) & -151.19363  & -151.195266 &             \\
F$_2$               & -199.0968(2)  & -199.0965(2) & -199.097448 & -199.099328 &             \\
CO$_2$              & -188.1561(2)  & -188.1525(2) & -188.147429 &             & -188.149551 \\ \hline 
RMSD (in \unit{\milli \hartree}) &  2.89   &  2.73    & 1.65   & \\
MSD (in \unit{\milli \hartree})  &  -0.38  &  1.17    & 1.39   & \\
MAD (in \unit{\milli \hartree})  &  1.85   &  1.84    & 1.39    & \\
\end{tabular}
\end{ruledtabular}
\end{table*}

==> tables/w_clusters.tex <==
\begin{table*}
\caption{\label{tab:wclusters} Binding energies of the four most stable water clusters containing up to 5 H$_2$O molecules calculated using heavy-augmented cc-pVDZ basis set and  all-electron wavefunctions. RHF, MP2, CCSD(T), and different ph-AFQMC values in $\unit{\kilo \cal / \mole}$ are reported.}
\begin{ruledtabular}
\begin{tabular}{l*{6}{d}}
Cluster             & \multicolumn{1}{c}{RHF }& \multicolumn{1}{c}{MP2} & \multicolumn{1}{c}{CCSD(T)} & \multicolumn{1}{c}{ph-AFQMC} & \multicolumn{1}{c}{ph$^{*}$-AFQMC} & \multicolumn{1}{c}{ph-AFQMC\cite{Motta2109-AFQMC-ED}} \\ \hline
2Cs                 & -3.82    & -5.22    & -5.18   & -5.17(5)    & -5.06(7)    &  -5.11(31)        \\
3UUD                & -10.52   & -15.83   & -15.62  & -15.67(9)   & -15.68(9)   &  -14.78(64)       \\
4S4                 & -19.00   & -28.36   & -27.87  & -28.12(10)  & -28.11(10)  &  -26.49(46)       \\
5CYC                & -25.30   & -37.48   & -36.78  & -37.14(28)  & -37.31(28)  &  -36.27(59)       \\ 
\end{tabular}
\end{ruledtabular}
\end{table*}
